On Trapped Modes In Variable White Dwarfs As Probes Of The $^{12}$C($\alpha, \gamma$)$^{16}$O Reaction Rate

We seek signatures of the current experimental $^{12}$C$(\alpha,\gamma)^{16}$O reaction rate probability distribution function in the pulsation periods of carbon-oxygen white dwarf models. We find that adiabatic g-modes trapped by the interior carbon-rich layer offer potentially useful signatures of this reaction rate probability distribution function. Probing the carbon-rich region is relevant because it forms during the evolution of low-mass stars under radiative helium burning conditions, mitigating the impact of convective mixing processes. We make direct quantitative connections between the pulsation periods of the identified trapped g-modes in variable WD models and the current experimental $^{12}$C$(\alpha,\gamma)^{16}$O reaction rate probability distribution function. We find an average spread in relative period shifts of $\Delta P/P \simeq \pm$ 2\% for the identified trapped g-modes over the $\pm$ 3$\sigma$ uncertainty in the $^{12}$C$(\alpha,\gamma)^{16}$O reaction rate probability distribution function -- across the effective temperature range of observed DAV and DBV white dwarfs and for different white dwarf masses, helium shell masses, and hydrogen shell masses. The g-mode pulsation periods of observed white dwarfs are typically given to 6-7 significant figures of precision. This suggests that an astrophysical constraint on the $^{12}$C$(\alpha,\gamma)^{16}$O reaction rate could, in principle, be extractable from the period spectrum of observed variable white dwarfs.

==> vectors.tex <==
%=======================================================================
%
% vectors.tex---some basic vector operators
%
% Requires package bm.sty
%
%=======================================================================

\RequirePackage{bm}
%\RequirePackage{amssymb}
%\RequirePackage{amsbsy}
\newcommand{\bvec}[1]{\ensuremath{\boldsymbol{#1}}} %boldface vector style
\newcommand{\grad}{\bvec{\nabla}} %gradient
\newcommand{\divr}{\bvec{\nabla} \cdot} %divergence
\newcommand{\curl}{\bvec{\nabla \times}} %curl
\newcommand{\lap}{\ensuremath{\nabla^2}} %Laplacian
\newcommand{\btens}[1]{\ensuremath{\boldsymbol{\mathsf{#1}}}}
\newcommand{\vcross}{\bvec{\times}}
\newcommand{\vdot}{\bvec{\cdot}}
% end vectors.tex
